Multi-Agent Safe Planning with Gaussian Processes

Multi-agent safe systems have become an increasingly important area of study as we can now easily have multiple AI-powered systems operating together. In such settings, we need to ensure the safety of not only each individual agent, but also the overall system. In this paper, we introduce a novel multi-agent safe learning algorithm that enables decentralized safe navigation when there are multiple different agents in the environment. This algorithm makes mild assumptions about other agents and is trained in a decentralized fashion, i.e. with very little prior knowledge about other agents' policies. Experiments show our algorithm performs well with the robots running other algorithms when optimizing various objectives.

==> sections/conclusion.tex <==
In this paper, we presented the decentralized planning algorithm, Multi-agent SafeMDP, that allows agents to avoid stepping into unsafe states with a GP approach and avoid experiencing jointly unsafe conditions. This algorithm assumes no prior knowledge on other agents and learns other agents' policies through observations. We showed that the algorithm has polynomial time complexity in the sizes of state space, action space, and the number of the agents. We also gave a performance guarantee on the exploitation policy estimate on other agents. We empirically show with our experiments that the algorithm works well with the agents of the same kind or the agents that employ other standard algorithms.
